Loop Closure Prioritization for Efficient and Scalable Multi-Robot SLAM

Multi-robot SLAM systems in GPS-denied environments require loop closures to maintain a drift-free centralized map. With an increasing number of robots and size of the environment, checking and computing the transformation for all the loop closure candidates becomes computationally infeasible. In this work, we describe a loop closure module that is able to prioritize which loop closures to compute based on the underlying pose graph, the proximity to known beacons, and the characteristics of the point clouds. We validate this system in the context of the DARPA Subterranean Challenge and on numerous challenging underground datasets and demonstrate the ability of this system to generate and maintain a map with low error. We find that our proposed techniques are able to select effective loop closures which results in 51% mean reduction in median error when compared to an odometric solution and 75% mean reduction in median error when compared to a baseline version of this system with no prioritization. We also find our proposed system is able to find a lower error in the mission time of one hour when compared to a system that processes every possible loop closure in four and a half hours. The code and dataset for this work can be found https://github.com/NeBula-Autonomy/LAMP

==> tables/computation_test.tex <==
\begin{table*}
\centering
\caption{We perform the experiments with limited computation and compare the results between the old method and the new. \yc{Maybe get rid of this and merge with Figure 5. }}
\begin{tabular}{@{}rrrrcrrrcrrr@{}}
\hline
& \multicolumn{4}{c}{LAMP 1.0} & \phantom{abc}& \multicolumn{4}{c}{LAMP 2.0} \\
\cline{2-5} \cline{7-10}
& Detected & Inlier Ratio & Odom APE & APE && Detected & Inlier Ratio & Odom APE & APE\\ 
\hline
KU \\
H1 & 0 & 0 & 0 & 0 && 0 & 0 & 0 & 0\\
H2 & 0 & 0 & 0 & 0 && 0 & 0 & 0 & 0\\
S1 & 0 & 0 & 0 & 0 && 0 & 0 & 0 & 0\\
S2 & 0 & 0 & 0 & 0 && 0 & 0 & 0 & 0\\
\hline
Final \\
H1 & 0 & 0 & 0 & 0 && 0 & 0 & 0 & 0\\
H2 & 0 & 0 & 0 & 0 && 0 & 0 & 0 & 0\\
S1 & 0 & 0 & 0 & 0 && 0 & 0 & 0 & 0\\
S2 & 0 & 0 & 0 & 0 && 0 & 0 & 0 & 0\\
\hline
\end{tabular}
\end{table*}

==> tables/superbase_comparison_table.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t!]
\centering
\caption{Comparison of different loop candidate selection methods (Superbase) }\label{tab:lc-ablation}
\begin{tabular}{cl cccccc}
\toprule
& & \multicolumn{4}{c}{\# of Loop Closures} \\
\midrule
& & Candidates & Selected & Verified & GNC-Inliers & Inliers & ATE \\
\midrule
\multirow{4}{*}{Tunnel}
& Baseline & 0 & 23177 & 3178 & 626 & 971 & 1.53 \\
& Obs & 8839 & 6638 & 4172 & 3059 & 3161 & 0.88 \\
& R.Btr & 9744 & 9500 & 5032 & 3438 & 3462 & 0.84 \\
& Btr & 9419 & 9000 & 5016 & 3531 & 3507 & 0.83 \\
& Full & 9754 & 9427 & 5695 & 3760 & 4085 & 0.78 \\
\midrule
\multirow{4}{*}{Urban}
& Baseline & 0 & 17633 & 515 & 79 & 58 & 0.99 \\
& Obs & 5307 & 4847 & 1612 & 549 & 572 & 1.14 \\
& R.Btr & 5239 & 5000 & 1609 & 795 & 630 & 0.98 \\
& Btr & 5561 & 5500 & 1819 & 807 & 885 & 0.96 \\
& Full & 5336 & 4880 & 1604 & 561 & 555 & 1.94 \\
\midrule
\multirow{4}{*}{KU}
& Baseline & 0 & 23020 & 12 & 5 & 1 & 4.29 \\
& Obs & 22332 & 22314 & 850 & 418 & 374 & 1.51 \\
& R.Btr & 21053 & 21000 & 742 & 455 & 376 & 2.01 \\
& Btr & 22315 & 22000 & 680 & 399 & 282 & 1.66 \\
& Full & 22283 & 22268 & 850 & 434 & 375 & 1.15 \\
\midrule
\multirow{4}{*}{Final}
& Baseline & 0 & 12702 & 723 & 37 & 67 & 0.63 \\
& Obs & 2671 & 2016 & 827 & 438 & 520 & 0.19 \\
& R.Btr & 3867 & 3500 & 1265 & 554 & 757 & 0.38 \\
& Btr & 2573 & 2500 & 829 & 600 & 511 & 0.43 \\
& Full & 3854 & 3755 & 1487 & 507 & 787 & 0.29 \\
\end{tabular}
\end{table}
